Filters for X-ray detectors on Space missions

Thin filters and gas tight windows are used in Space to protect sensitive X-ray detectors from out-of-band electromagnetic radiation, low-energy particles, and molecular contamination. Though very thin and made of light materials, filters are not fully transparent to X-rays. For this reason, they ultimately define the detector quantum efficiency at low energies. In this chapter, we initially provide a brief overview of filter materials and specific designs adopted on space experiments with main focus on detectors operating at the focal plane of grazing incidence X-ray telescopes. We then provide a series of inputs driving the design and development of filters for high-energy astrophysics space missions. We begin with the identification of the main functional goals and requirements driving the preliminary design, and identify modeling tools and experimental characterization techniques needed to prove the technology and consolidate the design. Finally, we describe the calibration activities required to derive the filter response with high accuracy.We conclude with some hints on materials and technologies presently under investigation for future X-ray missions.

==> content_notes.tex <==

\textbf{CONTENTS}
\begin{itemize}
\item Introduction (1 p.)(\textbf{Marco})
    \begin{itemize}
    \item filter purpose (thermal shields, optical blocking, RF attenuation, pass band, molecular contamination) 
    \item requirements (high x-ray transparency, low fluorescence yield, mechanical robustness, radiation hard, atomic oxygen resistent) in relazione alla tecnologia del rivelatore utilizzaato
    \item scope of the review (only x-ray detectors), chapter structure 
    \end{itemize}
\item Overview of filters in x-ray missions (3 p.)(\textbf{Marco})
    \begin{itemize}
    \item Einstein, EXOSAT, ROSAT,  Astro-D (ASCA), Beppo-SAX, Chandra, XMM, Astro-E, Astro-E2 (Suzaku), Astro-H (Hitomi), E-Rosita, XRISM-resolve, Athena, Lynx, Arcus in aggiunta cenno a esperimenti solari e.g. Solar-A/Johkoh , Solar-B/Hinode)
    \item Fig.1 - confronto trasmissione microcalorimeters detectors;  
    \end{itemize}
\item Requirements and Design Drivers (2 p.)(\textbf{Marco})
\item Filter Materials and Technologies (3 p.)(\textbf{Marco}) - anche elenco aziende produttrici in ambito spaziale
\item Performance Modeling (3 p.)(\textbf{Ugo}) (x-ray transmission (photoelectric cross section ma anche scattering, compton, Bragg per filtri più spessi e per energie maggiori 10 keV), strutture fini di assorbimento (Luisa darà un contributo sul significato delle strutture da un punto di vista strutturale), out of band attenuation, mechanical, thermal) 
\item Characterization techniques (7 p.)
    \begin{itemize}
    \item Cappello introduttivo (0.5 p) (\textbf{Marco})  
    \item  XPS (1 p.) (\textbf{Luisa})
    \item  X-ray transmission Spectroscopy and Imaging (1 p.) (\textbf{Luisa})
    \item UV/VIS/IR Spectroscopy (1 p.) (\textbf{Luisa})
    \item  Radiofrequency (1 p.) (\textbf{Ugo})
    \item Imaging (0.5 p.) ((AFM, SEM, Microscopia Ottica e  IR, photographic scanner) (\textbf{Luisa})
    \item Aging in space environment  (Radiation damage/atomic oxygen/micro-meteoroids) (1 p.) (\textbf{Marco/Ugo})
    \item Mechanical loads (static and vibro-acoustics) (1.p) (\textbf{Marco)}
    \item Thermo-vacuum, moisture stress (0.5 p.) (\textbf{Ugo})
    \end{itemize}
\item Calibration (methodology, accuracy, experimental set-up) (2 p.) (\textbf{Luisa})
\item Future perspectives (new technologies, meshes, future missions) (2 p.) (\textbf{Marco, ...})
\item References

\end{itemize}
